Beehive: A Flexible Network Stack for Direct-Attached Accelerators

Direct-attached accelerators, where application accelerators are directly connected to the datacenter network via a hardware network stack, offer substantial benefits in terms of reduced latency, CPU overhead, and energy use. However, a key challenge is that modern datacenter network stacks are complex, with interleaved protocol layers, network management functions, and virtualization support. To operators, network feature agility, diagnostics, and manageability are often considered just as important as raw performance. By contrast, existing hardware network stacks only support basic protocols and are often difficult to extend since they use fixed processing pipelines. We propose Beehive, a new, open-source FPGA network stack for direct-attached accelerators designed to enable flexible and adaptive construction of complex network functionality in hardware. Application and network protocol elements are modularized as tiles over a network-on-chip substrate. Elements can be added or scaled up/down to match workload characteristics with minimal effort or changes to other elements. Flexible diagnostics and control are integral, with tooling to ensure deadlock safety. Our implementation interoperates with standard Linux TCP and UDP clients, with a 4x improvement in end-to-end RPC tail latency for Linux UDP clients versus a CPU-attached accelerator. Beehive is available at https://github.com/beehive-fpga/beehive

==> figs/micro_latency_table.tex <==
\begin{table}[h]
\begin{tabular}{lll}
                   & Beehive & No NoC \\ 
\cline{2-3} 
Stack Latency (ns) & 392     & 224   
\end{tabular}
\end{table}

==> figs/rs_energy_6k.tex <==
\begin{table}[]
    \centering
    \footnotesize
    \caption{Energy consumption and goodput for Reed-Solomon encoding using
    Beehive versus CPU for 1, 2, 3 and 4 application instances and (6K, 1K)}
\begin{tabular}{lllll}
                                            & 1 app & 2 app & 3 app & 4 app \\
\toprule                               
\multicolumn{1}{l|}{CPU Energy (mj/op)}     & 1.47  & 0.630 & 0.424 & 0.403 \\
\multicolumn{1}{l|}{Beehive Energy (mj/op)} & 0.051 & 0.028 & 0.020 & 0.017 \\
\cline{2-5}
\multicolumn{1}{l|}{Energy efficiency}      & 28.8x & 22.5x & 21.2x & 23.7x \\
\midrule
\multicolumn{1}{l|}{CPU Goodput (Gbps)}     & 2.64  & 6.46  & 9.28  & 11.1  \\
\multicolumn{1}{l|}{Beehive Goodput (Gbps)} & 27.0  & 53.9  & 80.8  & 99.1  \\
\cline{2-5}
\multicolumn{1}{l|}{Speedup}                & 10.2x & 8.34x & 8.71x & 8.93  \\
\bottomrule
\end{tabular}
\end{table}

==> figs/rs_scalability_table.tex <==
\begin{table}[h]
    \centering  
    \footnotesize
    \caption{Aggregate goodput of the FPGA server as we scale up the number of
    Reed-Solomon encoder instances. The goodput scales linearly as we add more
    instances. \fixme{Should be line graph with CPU comparison}}
    \resizebox{\linewidth}{!}
    {    
        \begin{tabular}{lllll}
        \# of instances       & 1      & 2      & 3       & 4       \\
        \hline
        \multicolumn{1}{l|}{Goodput (Gbps)} & 26.95  & 53.89  & 80.84   & 99.31   \\
        \multicolumn{1}{l|}{MReqs/sec}      & 0.4699 & 0.9398 & 1.4097 & 1.7320    
        \end{tabular}
    }
    \label{tab:rs_encode_scaling}
\end{table}

==> rel_work_table.tex <==
\newcommand\greenfull{%
  \begin{tikzpicture}
    \draw[green, fill] (0,0) circle (1ex);
  \end{tikzpicture}%
}
\newcommand\bluepartial[1][1ex]{%
  \begin{tikzpicture}
  \draw[fill, blue] (0,0)-- (90:#1) arc (90:270:#1) -- cycle ;
  \draw[thick, blue] (0,0) circle (#1);
  \end{tikzpicture}}
\newcommand\redempty{%
  \begin{tikzpicture}
    \draw[red, thick] (0,0) circle (1ex);
  \end{tikzpicture}%
  
}

\begin{table*}[t]
\centering
\begin{tabular}{lccccccc}
\toprule
 & Standard Protocols & Modularity & Scalability & Performance & Management Features & Open-source & Language(s)\\
\midrule
HLS TCP engine~\cite{limago} & \greenfull & \bluepartial & \redempty & \greenfull & \redempty & \greenfull & Vitis HLS \& Verilog\\
PANIC~\cite{panic_osdi} & \bluepartial & \greenfull & \redempty & \greenfull & \redempty & \greenfull & Verilog \\
ClickNP~\cite{clicknp_sigcomm} & \bluepartial & \greenfull & \bluepartial & \greenfull & \greenfull & \redempty & N/A \\
Microsoft LTL~\cite{catapult_v2} & \redempty & \redempty & \bluepartial & \greenfull & \redempty & \redempty & N/A \\
\thesystem & \greenfull & \greenfull & \greenfull & \greenfull & \greenfull & \greenfull & SystemVerilog \\


\hline
\end{tabular}
\caption{Related work comparisons}
\label{tab:rel_work_comparison}
\end{table*}

==> rev_relwork.tex <==
As shown in Table~\ref{tab:rel_work_table}, other related work does not meet all these goals. 
In terms of complexity, the Limago, a TCP engine written in Vitis HLS, is the closest to \thesystem.
However, it is not designed to allow for addition or replication of components within the stack, so it is limited in scalability and modularity. We discuss FPGA utilization comparisons further in Section \ref{sec:hw_util}. Unfortunately, we were unable to run Limago on our FPGAs using their code~\cite{limago_build_repo} to evaluate its performance, because the QSFPs did not come up on the FPGA board.

PANIC and ClickNP are the most similar architecturally to \thesystem as they are both based on message-passing over an interconnect, leading to similar performance and modularity benefits as \thesystem. 
Their implementations do not provide standard protocol support directly, but they could be extended to support the logic needed for these protocols.
More importantly, their interconnects can limit their scalability. While working on the experiment in Section \ref{sec:beehive_udp_microbench}, we found PANIC's crossbar was unable to support more than 8 endpoints, 4 of which are always used by its infrastructure. In ClickNP, components are directly connected using FIFOs, potentially causing fan-out issues when duplicating components. Because ClickNP is not open-source, we were unable to compare to it directly. 

